Information-Theoretic Probing with Minimum Description Length

To measure how well pretrained representations encode some linguistic property, it is common to use accuracy of a probe, i.e. a classifier trained to predict the property from the representations. Despite widespread adoption of probes, differences in their accuracy fail to adequately reflect differences in representations. For example, they do not substantially favour pretrained representations over randomly initialized ones. Analogously, their accuracy can be similar when probing for genuine linguistic labels and probing for random synthetic tasks. To see reasonable differences in accuracy with respect to these random baselines, previous work had to constrain either the amount of probe training data or its model size. Instead, we propose an alternative to the standard probes, information-theoretic probing with minimum description length (MDL). With MDL probing, training a probe to predict labels is recast as teaching it to effectively transmit the data. Therefore, the measure of interest changes from probe accuracy to the description length of labels given representations. In addition to probe quality, the description length evaluates "the amount of effort" needed to achieve the quality. This amount of effort characterizes either (i) size of a probing model, or (ii) the amount of data needed to achieve the high quality. We consider two methods for estimating MDL which can be easily implemented on top of the standard probing pipelines: variational coding and online coding. We show that these methods agree in results and are more informative and stable than the standard probes.

==> jiant_code_figures.tex <==




\begin{figure*}[t!]
    \centering
    \subfloat[POS]
    {\includegraphics[scale=0.26]{pict/jiant_by_type_pos.png}}
    \quad
    \subfloat[Constituents]
    {\includegraphics[scale=0.26]{pict/jiant_by_type_nonterm_.png}}
    \quad
    \subfloat[Dependencies]
    {\includegraphics[scale=0.26]{pict/jiant_by_type_dep_.png}}
    \quad
    \subfloat[Entities]
    {\includegraphics[scale=0.26]{pict/jiant_by_type_ner_.png}}
    %\quad
    \\
    \subfloat[SRL]
    {\includegraphics[scale=0.26]{pict/jiant_by_type_srl.png}}
    \quad
    \subfloat[Coreference]
    {\includegraphics[scale=0.26]{pict/jiant_by_type_coref_.png}}
    \quad
    \subfloat[Rel. (SemEval)]
    {\includegraphics[scale=0.26]{pict/jiant_by_type_relsem_.png}}
    \quad
    %\subfloat[Entities]
    {\includegraphics[scale=0.26]{pict/data_model_legend.png}}
    \quad

    \caption{Codelength split into data and model codes.}
    \label{fig:by_type_jiant}
\end{figure*}

==> jiant_main_table.tex <==

% \begin{table*}[t!]
% \centering
% \begin{tabular}{lcccccc}
% \toprule
% %& \multicolumn{3}{c}{segmentation}\\
%  & & \bf Accuracy  & \multicolumn{4}{c}{\bf Description Length}\\
%  & &   & \multicolumn{2}{c}{\bf variational code}  & \multicolumn{2}{c}{\bf online code} \\
%  & &    &  codelength & compression & codelength & compression \\
% \midrule
% \multicolumn{5}{l}{\!\!\!\bf Part-of-speech}\\
% & layer 0 & 90.9 / - & 483 / - & 23.4 / -  & 479 / - & 23.6 / -  \\
% & layer 1 & 97.3 / 94.8 &  209 / 273 & 54.0 / 41.4  & 218 / 356 & 51.85 / 31.76  \\
% & layer 2 & 96.7 / 94.7 & 252 / 273 & 44.7 / 41.4  & 260 / 356 & 43.35 / 31.74  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Constituents}\\
% & layer 0 & 74.4 / - &  1181 / - & 7.5 / -  & 1229 / - & 7.2 / -  \\
% & layer 1 & 84.7 / 75.7 &  603 / 877 & 14.7 / 10.1  & 663 / 1184 & 13.38 / 7.49  \\
% & layer 2 & 82.6 / 75.8 &  719 / 875 & 12.3 / 10.1  & 800 / 1179 & 11.1 / 7.52  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Dependencies}\\
% & layer 0 & 78.4 / - &  158 / - & 7.1 / -  & 186 / - & 6.0 / -  \\
% & layer 1 & 91.7 / 87.9 &  80 / 103 & 14.0 / 10.8  & 82 / 125 & 13.65 / 8.93  \\
% & layer 2 & 90.5 / 88.2 &  94 / 103 & 11.9 / 10.8  & 91 / 125 & 12.25 / 8.94  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Entities}\\
% & layer 0 &  92.2 / - &  40 / - & 13.2 / -   &  40 / - & 13.3 / -  \\
% & layer 1 & 94.3 / 92.7 &   27 / 34 & 19.3 / 15.4   & 28 / 38 & 18.52 / 13.95  \\
% & layer 2 & 94.5 / 92.8 &   30 / 34 & 17.7 / 15.2   & 28 / 38 & 18.82 / 13.92  \\
% \midrule

% \multicolumn{5}{l}{\!\!\!\bf SRL}\\
% & layer 0 & 78.9 / -  &  411 / - & 8.6 / -  & 410 / - & 8.6 / -  \\
% & layer 1 &   89.5 / 82.5   & 228 / 306 & 15.5 / 11.5   & 236 / 388 & 14.97 / 9.12  \\
% & layer 2 &  87.9 / 82.9  & 272 / 306 & 13.0 / 11.6   & 272 / 387 & 13.0 / 9.14  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Coreference}\\
% & layer 0 & 89.0 / - & 57.4 / - & 3.54 / -  & 62 / - & 3.3 / -  \\
% & layer 1 & 91.7 / 89.6 &  50.3 / 54.5 & 4.04 / 3.72  & 56 / 69 & 3.6 / 2.95  \\
% & layer 2 & 90.3 / 89.7 &  56.8 / 54.3 & 3.57 / 3.74  & 63 / 69 & 3.2 / 2.93  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Rel. (SemEval)}\\
% & layer 0 & 51.6 / - &  11.5 / - & 2.48 / -   &  14.4 / - & 1.97 / -   \\
% & layer 1 & 71.0 / 64.3 &  8.0 / 9.7 & 3.56 / 2.94   & 7.9 / 10.8 & 3.6 / 2.62  \\
% & layer 2 & 73.6 / 64.4  &  8.4 / 9.7 & 3.40 / 2.92   &  7.9 / 10.7 & 3.62 / 2.65  \\

% \bottomrule
% \end{tabular}
% \caption{base/random. codelength - in kbits}
% \label{tab:main}
% \end{table*}





\begin{table*}[t!]
\centering
\begin{tabular}{lcccccc}
\toprule
%& \multicolumn{3}{c}{segmentation}\\
 & & \bf Accuracy  & \multicolumn{4}{c}{\bf Description Length}\\
 & &   & \multicolumn{2}{c}{\bf variational code}  & \multicolumn{2}{c}{\bf online code} \\
 & &    &  codelength & compression & codelength & compression \\
\midrule
\multicolumn{5}{l}{\!\!\!\bf Part-of-speech}\\
& layer 0 & 90.9 & 483 & 23.4  & 479 & 23.6  \\
& layer 1 & 97.3 / 94.8 &  209 / 273 & 54.0 / 41.4  & 218 / 356 & 51.85 / 31.76  \\
& layer 2 & 96.7 / 94.7 & 252 / 273 & 44.7 / 41.4  & 260 / 356 & 43.35 / 31.74  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Constituents}\\
& layer 0 & 74.4 &  1181 & 7.5  & 1229  & 7.2   \\
& layer 1 & 84.7 / 75.7 &  603 / 877 & 14.7 / 10.1  & 663 / 1184 & 13.38 / 7.49  \\
& layer 2 & 82.6 / 75.8 &  719 / 875 & 12.3 / 10.1  & 800 / 1179 & 11.1 / 7.52  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Dependencies}\\
& layer 0 & 78.4 &  158  & 7.1  & 186  & 6.0   \\
& layer 1 & 91.7 / 87.9 &  80 / 103 & 14.0 / 10.8  & 82 / 125 & 13.65 / 8.93  \\
& layer 2 & 90.5 / 88.2 &  94 / 103 & 11.9 / 10.8  & 91 / 125 & 12.25 / 8.94  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Entities}\\
& layer 0 &  92.2  &  40  & 13.2    &  40 & 13.3  \\
& layer 1 & 94.3 / 92.7 &   27 / 34 & 19.3 / 15.4   & 28 / 38 & 18.52 / 13.95  \\
& layer 2 & 94.5 / 92.8 &   30 / 34 & 17.7 / 15.2   & 28 / 38 & 18.82 / 13.92  \\
\midrule

\multicolumn{5}{l}{\!\!\!\bf SRL}\\
& layer 0 & 78.9   &  411  & 8.6   & 410  & 8.6   \\
& layer 1 &   89.5 / 82.5   & 228 / 306 & 15.5 / 11.5   & 236 / 388 & 14.97 / 9.12  \\
& layer 2 &  87.9 / 82.9  & 272 / 306 & 13.0 / 11.6   & 272 / 387 & 13.0 / 9.14  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Coreference}\\
& layer 0 & 89.0  & 57.4  & 3.54   & 62  & 3.3   \\
& layer 1 & 91.7 / 89.6 &  50.3 / 54.5 & 4.04 / 3.72  & 56 / 69 & 3.6 / 2.95  \\
& layer 2 & 90.3 / 89.7 &  56.8 / 54.3 & 3.57 / 3.74  & 63 / 69 & 3.2 / 2.93  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Rel. (SemEval)}\\
& layer 0 & 51.6  &  11.5  & 2.48    &  14.4  & 1.97    \\
& layer 1 & 71.0 / 64.3 &  8.0 / 9.7 & 3.56 / 2.94   & 7.9 / 10.8 & 3.60 / 2.62  \\
& layer 2 & 73.6 / 64.4  &  8.4 / 9.7 & 3.40 / 2.92   &  7.9 / 10.7 & 3.62 / 2.65  \\

\bottomrule
\end{tabular}
\caption{base/random. codelength - in kbits}
\label{tab:jiant_main}
\end{table*}


==> jiant_main_table_old.tex <==

% \begin{table*}[t!]
% \centering
% \begin{tabular}{lcccccc}
% \toprule
% %& \multicolumn{3}{c}{segmentation}\\
%  & & \bf Accuracy  & \multicolumn{4}{c}{\bf Description Length}\\
%  & &   & \multicolumn{2}{c}{\bf variational code}  & \multicolumn{2}{c}{\bf online code} \\
%  & &    &  codelength & compression & codelength & compression \\
% \midrule
% \multicolumn{5}{l}{\!\!\!\bf Part-of-speech}\\
% & layer 0 & 90.9 / - & 483 / - & 23.4 / -  & 479 / - & 23.6 / -  \\
% & layer 1 & 97.3 / 94.8 &  209 / 273 & 54.0 / 41.4  & 218 / 356 & 51.85 / 31.76  \\
% & layer 2 & 96.7 / 94.7 & 252 / 273 & 44.7 / 41.4  & 260 / 356 & 43.35 / 31.74  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Constituents}\\
% & layer 0 & 74.4 / - &  1181 / - & 7.5 / -  & 1229 / - & 7.2 / -  \\
% & layer 1 & 84.7 / 75.7 &  603 / 877 & 14.7 / 10.1  & 663 / 1184 & 13.38 / 7.49  \\
% & layer 2 & 82.6 / 75.8 &  719 / 875 & 12.3 / 10.1  & 800 / 1179 & 11.1 / 7.52  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Dependencies}\\
% & layer 0 & 78.4 / - &  158 / - & 7.1 / -  & 186 / - & 6.0 / -  \\
% & layer 1 & 91.7 / 87.9 &  80 / 103 & 14.0 / 10.8  & 82 / 125 & 13.65 / 8.93  \\
% & layer 2 & 90.5 / 88.2 &  94 / 103 & 11.9 / 10.8  & 91 / 125 & 12.25 / 8.94  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Entities}\\
% & layer 0 &  92.2 / - &  40 / - & 13.2 / -   &  40 / - & 13.3 / -  \\
% & layer 1 & 94.3 / 92.7 &   27 / 34 & 19.3 / 15.4   & 28 / 38 & 18.52 / 13.95  \\
% & layer 2 & 94.5 / 92.8 &   30 / 34 & 17.7 / 15.2   & 28 / 38 & 18.82 / 13.92  \\
% \midrule

% \multicolumn{5}{l}{\!\!\!\bf SRL}\\
% & layer 0 & 78.9 / -  &  411 / - & 8.6 / -  & 410 / - & 8.6 / -  \\
% & layer 1 &   89.5 / 82.5   & 228 / 306 & 15.5 / 11.5   & 236 / 388 & 14.97 / 9.12  \\
% & layer 2 &  87.9 / 82.9  & 272 / 306 & 13.0 / 11.6   & 272 / 387 & 13.0 / 9.14  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Coreference}\\
% & layer 0 & 89.0 / - & 57.4 / - & 3.54 / -  & 62 / - & 3.3 / -  \\
% & layer 1 & 91.7 / 89.6 &  50.3 / 54.5 & 4.04 / 3.72  & 56 / 69 & 3.6 / 2.95  \\
% & layer 2 & 90.3 / 89.7 &  56.8 / 54.3 & 3.57 / 3.74  & 63 / 69 & 3.2 / 2.93  \\

% \midrule

% \multicolumn{5}{l}{\!\!\!\bf Rel. (SemEval)}\\
% & layer 0 & 51.6 / - &  11.5 / - & 2.48 / -   &  14.4 / - & 1.97 / -   \\
% & layer 1 & 71.0 / 64.3 &  8.0 / 9.7 & 3.56 / 2.94   & 7.9 / 10.8 & 3.6 / 2.62  \\
% & layer 2 & 73.6 / 64.4  &  8.4 / 9.7 & 3.40 / 2.92   &  7.9 / 10.7 & 3.62 / 2.65  \\

% \bottomrule
% \end{tabular}
% \caption{base/random. codelength - in kbits}
% \label{tab:main}
% \end{table*}





\begin{table*}[t!]
\centering
\begin{tabular}{lcccccc}
\toprule
%& \multicolumn{3}{c}{segmentation}\\
 & & \bf Accuracy  & \multicolumn{4}{c}{\bf Description Length}\\
 & &   & \multicolumn{2}{c}{\bf variational code}  & \multicolumn{2}{c}{\bf online code} \\
 & &    &  codelength & compression & codelength & compression \\
\midrule
\multicolumn{5}{l}{\!\!\!\bf Part-of-speech}\\
& layer 0 & 90.9 & 483 & 23.4  & 479 & 23.6  \\
& layer 1 & 97.3 / 94.8 &  209 / 273 & 54.0 / 41.4  & 218 / 356 & 51.85 / 31.76  \\
& layer 2 & 96.7 / 94.7 & 252 / 273 & 44.7 / 41.4  & 260 / 356 & 43.35 / 31.74  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Constituents}\\
& layer 0 & 74.4 &  1181 & 7.5  & 1229  & 7.2   \\
& layer 1 & 84.7 / 75.7 &  603 / 877 & 14.7 / 10.1  & 663 / 1184 & 13.38 / 7.49  \\
& layer 2 & 82.6 / 75.8 &  719 / 875 & 12.3 / 10.1  & 800 / 1179 & 11.1 / 7.52  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Dependencies}\\
& layer 0 & 78.4 &  158  & 7.1  & 186  & 6.0   \\
& layer 1 & 91.7 / 87.9 &  80 / 103 & 14.0 / 10.8  & 82 / 125 & 13.65 / 8.93  \\
& layer 2 & 90.5 / 88.2 &  94 / 103 & 11.9 / 10.8  & 91 / 125 & 12.25 / 8.94  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Entities}\\
& layer 0 &  92.2  &  40  & 13.2    &  40 & 13.3  \\
& layer 1 & 94.3 / 92.7 &   27 / 34 & 19.3 / 15.4   & 28 / 38 & 18.52 / 13.95  \\
& layer 2 & 94.5 / 92.8 &   30 / 34 & 17.7 / 15.2   & 28 / 38 & 18.82 / 13.92  \\
\midrule

\multicolumn{5}{l}{\!\!\!\bf SRL}\\
& layer 0 & 78.9   &  411  & 8.6   & 410  & 8.6   \\
& layer 1 &   89.5 / 82.5   & 228 / 306 & 15.5 / 11.5   & 236 / 388 & 14.97 / 9.12  \\
& layer 2 &  87.9 / 82.9  & 272 / 306 & 13.0 / 11.6   & 272 / 387 & 13.0 / 9.14  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Coreference}\\
& layer 0 & 89.0  & 57.4  & 3.54   & 62  & 3.3   \\
& layer 1 & 91.7 / 89.6 &  50.3 / 54.5 & 4.04 / 3.72  & 56 / 69 & 3.6 / 2.95  \\
& layer 2 & 90.3 / 89.7 &  56.8 / 54.3 & 3.57 / 3.74  & 63 / 69 & 3.2 / 2.93  \\

\midrule

\multicolumn{5}{l}{\!\!\!\bf Rel. (SemEval)}\\
& layer 0 & 51.6  &  11.5  & 2.48    &  14.4  & 1.97    \\
& layer 1 & 71.0 / 64.3 &  8.0 / 9.7 & 3.56 / 2.94   & 7.9 / 10.8 & 3.60 / 2.62  \\
& layer 2 & 73.6 / 64.4  &  8.4 / 9.7 & 3.40 / 2.92   &  7.9 / 10.7 & 3.62 / 2.65  \\

\bottomrule
\end{tabular}
\caption{base/random. codelength - in kbits}
\label{tab:jiant_main}
\end{table*}

